Identity testing under label mismatch

Testing whether the observed data conforms to a purported model (probability distribution) is a basic and fundamental statistical task, and one that is by now well understood. However, the standard formulation, identity testing, fails to capture many settings of interest; in this work, we focus on one such natural setting, identity testing under promise of permutation. In this setting, the unknown distribution is assumed to be equal to the purported one, up to a relabeling (permutation) of the model: however, due to a systematic error in the reporting of the data, this relabeling may not be the identity. The goal is then to test identity under this assumption: equivalently, whether this systematic labeling error led to a data distribution statistically far from the reference model.

==> packages.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{bbm}
%
%
\usepackage{xspace}                                     %
%

%
%

%
\usepackage{amsfonts,amsmath,amssymb, amsthm, mathtools}
\usepackage{thm-restate}
\usepackage{dsfont} %

%
\usepackage{algorithmicx,algpseudocode,algorithm}

%
\usepackage[usenames,dvipsnames,table]{xcolor}

%
%

%
%

%
%

%
\usepackage{multirow}
%

%
\usepackage{mfirstuc}

%
\usepackage{tikz}
\usetikzlibrary{calc,plotmarks}
\usetikzlibrary{arrows}

%
\usepackage[colorlinks,citecolor=blue,bookmarks=true,linktocpage]{hyperref}
\usepackage{aliascnt}
\usepackage[numbered]{bookmark}
\usepackage[capitalise]{cleveref}

%
\usepackage{fullpage}

%
%

%
\usepackage[shortlabels]{enumitem}
%
%
%
   
%
\ifnum\withnotes=1
  \usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}
\fi

%
%

%
\usepackage{mleftright} %

\RequirePackage{pgfplots, tikz}
\pgfplotsset{compat=1.3}

\usepackage{tikz,forest}
\usetikzlibrary{arrows.meta}
\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}


==> preamble.tex <==
\makeatletter
\@ifundefined{theorem}{
  %
  \theoremstyle{plain} %
  	\newtheorem{theorem}{Theorem}[section]
  	\newtheorem*{theorem*}{Theorem} %
  	\newaliascnt{coro}{theorem}
  	  \newtheorem{corollary}[coro]{Corollary}
  	\aliascntresetthe{coro}
  	\newaliascnt{lem}{theorem}
  		\newtheorem{lemma}[lem]{Lemma}
  	\aliascntresetthe{lem}
  	\newaliascnt{clm}{theorem}
  		\newtheorem{claim}[clm]{Claim}
	\aliascntresetthe{clm}
	\newaliascnt{fact}{theorem}
 	 	\newtheorem{fact}[theorem]{Fact}
	\aliascntresetthe{fact}
  	\newtheorem*{unnumberedfact}{Fact}
  \newaliascnt{prop}{theorem}
  		\newtheorem{proposition}[prop]{Proposition}
	\aliascntresetthe{prop}
	\newaliascnt{conj}{theorem}
  		\newtheorem{conjecture}[conj]{Conjecture}
	\aliascntresetthe{conj}
 	 \newtheorem{problem}[theorem]{Problem}
  	\newtheorem{question}[theorem]{Question}
  	\newtheorem*{question*}{Question}
  \theoremstyle{remark} %
  	\newtheorem{remark}[theorem]{Remark}
  	\newtheorem*{notation}{Notation}
 	 \newtheorem{example}[theorem]{Example}
  \theoremstyle{definition} %
  	\newaliascnt{defn}{theorem}
 		 \newtheorem{definition}[defn]{Definition}
 	 \aliascntresetthe{defn}
 	 \newtheorem{observation}[theorem]{Observation}
 	 
 	 \newtheorem{openquestion}{Open Problem}
 	 \theoremstyle{plain}
 	 \newtheorem*{objective}{Goal}
}{}
%
\newtheorem{assumption}{Assumption}
\newenvironment{proofof}[1]{\begin{proof}[Proof of {#1}]}{\end{proof}}

\crefname{claim}{Claim}{Claims}

%
\providecommand{\email}[1]{\href{mailto:#1}{\nolinkurl{#1}\xspace}}

%
\ifnum\withcolors=1
  \newcommand{\new}[1]{{\color{red} {#1}}} %
  \newcommand{\newer}[1]{{\color{blue} {#1}}} %
  \newcommand{\newest}[1]{{\color{orange} {#1}}} %
  \newcommand{\newerest}[1]{{\color{blue!10!black!40!green} {#1}}} %
  \newcommand{\kcolor}[1]{{\color{ForestGreen}#1}} %
  \newcommand{\ccolor}[1]{{\color{RubineRed}#1}} %
\else
  \newcommand{\new}[1]{{{#1}}}
  \newcommand{\newer}[1]{{{#1}}}
  \newcommand{\newest}[1]{{{#1}}}
  \newcommand{\newerest}[1]{{{#1}}}
  \newcommand{\kcolor}[1]{{#1}}
  \newcommand{\ccolor}[1]{{#1}}
\fi
\renewcommand{\newerest}[1]{{\color{blue!10!black!40!green}{#1}}}
\ifnum\withnotes=1
  \newcommand{\knote}[1]{\par\kcolor{\textbf{K: }\scriptsize\sf #1}} %
  \newcommand{\cnote}[1]{\par\ccolor{\textbf{C: }\scriptsize\sf #1}} %
  \newcommand{\kfootnote}[1]{\footnote{{\bf \acolor{Karl}}: {#1}}}
  \newcommand{\cfootnote}[1]{\footnote{{\bf \ccolor{Cl\'ement}}: {#1}}}


  \newcommand{\todonote}[2][]{\todo[size=\tiny,color=red!40,#1]{#2}}  
	\newcommand{\questionnote}[2][]{\todo[size=\tiny,color=blue!30]{#2}}
	\newcommand{\todonotedone}[2][]{\todo[size=\tiny,color=green!40]{$\checkmark$ #2}}
	\newcommand{\todonoteinline}[2][]{\todo[inline,size=\tiny,color=orange!40,#1]{#2}}  
  \newcommand{\marginnote}[1]{\todo[size=\tiny,color=white,linecolor=black]{{#1}}}
\else
  \newcommand{\knote}[1]{}
  \newcommand{\cnote}[1]{}
  \newcommand{\todonote}[2][]{\ignore{#2}}
	\newcommand{\questionnote}[2][]{\ignore{#2}}
	\newcommand{\todonotedone}[2][]{\ignore{#2}}
	\newcommand{\todonoteinline}[2][]{\ignore{#2}}
  \newcommand{\marginnote}[1]{\ignore{#1}}
\fi
\newcommand{\ignore}[1]{\leavevmode\unskip} %
\newcommand{\kmargin}[1]{\questionnote{\kcolor{#1}}} %
\newcommand{\cmargin}[1]{\questionnote{\ccolor{#1}}} %

%
\newcommand{\eps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\Algo}{\ensuremath{\mathcal{A}}\xspace} %
\newcommand{\Tester}{\ensuremath{\mathcal{T}}\xspace} %
\newcommand{\Learner}{\ensuremath{\mathcal{L}}\xspace} %
\newcommand{\property}{\ensuremath{\mathcal{P}}\xspace} %
\newcommand{\task}{\ensuremath{\mathcal{P}}\xspace} %
\newcommand{\class}{\ensuremath{\mathcal{C}}\xspace} %
%
\newcommand{\eqdef}{:=}
\newcommand{\eqlaw}{\stackrel{\mathcal{L}}{=}}
\newcommand{\accept}{\textsf{accept}\xspace}
\newcommand{\fail}{\textsf{fail}\xspace}
\newcommand{\reject}{\textsf{reject}\xspace}
\newcommand{\opt}{{\textsc{opt}}\xspace}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\domain}{\ensuremath{\mathcal{X}}\xspace} %
\newcommand{\distribs}[1]{\Delta_{#1}} %
\newcommand{\yes}{{\sf{}yes}\xspace}
\newcommand{\no}{{\sf{}no}\xspace}
\newcommand{\dyes}{{\cal Y}}
\newcommand{\dno}{{\cal N}}

\newcommand{\Testing}{\ensuremath{\mathcal{T}}\xspace} %
\newcommand{\UTesting}{\ensuremath{\mathcal{T}^{\rm u}}\xspace} %
\newcommand{\Learning}{\ensuremath{\mathcal{L}}\xspace} %

%
\newcommand{\littleO}[1]{{o\mleft( #1 \mright)}}
\newcommand{\bigO}[1]{{O\mleft( #1 \mright)}}
\newcommand{\bigOSmall}[1]{{O\big( #1 \big)}}
\newcommand{\bigTheta}[1]{{\Theta\mleft( #1 \mright)}}
\newcommand{\bigOmega}[1]{{\Omega\mleft( #1 \mright)}}
\newcommand{\bigOmegaSmall}[1]{{\Omega\big( #1 \big)}}
\newcommand{\tildeO}[1]{\tilde{O}\mleft( #1 \mright)}
\newcommand{\tildeTheta}[1]{\operatorname{\tilde{\Theta}}\mleft( #1 \mright)}
\newcommand{\tildeOmega}[1]{\operatorname{\tilde{\Omega}}\mleft( #1 \mright)}
\providecommand{\poly}{\operatorname*{poly}}

%
\newcommand{\totinf}[1][f]{{\mathbf{Inf}[#1]}}
\newcommand{\infl}[2][f]{{\mathbf{Inf}_{#1}(#2)}}
\newcommand{\infldeg}[3][f]{{\mathbf{Inf}_{#1}^{#2}(#3)}}

%
\newcommand{\setOfSuchThat}[2]{ \left\{\; #1 \;\colon\; #2\; \right\} } 			%
\newcommand{\indicSet}[1]{\mathds{1}_{#1}}                                              %
\newcommand{\indic}[1]{\indicSet{\left\{#1\right\}}}                                             %
\newcommand{\disjunion}{\amalg}%

%
\newcommand{\dtv}{\operatorname{d}_{\rm TV}}
\newcommand{\hellinger}[2]{{\operatorname{d_{\rm{}H}}\mleft({#1, #2}\mright)}}
\newcommand{\kolmogorov}[2]{{\operatorname{d_{\rm{}K}}\mleft({#1, #2}\mright)}}
\newcommand{\totalvardistrestr}[3][]{{\dtv^{#1}\!\left({#2, #3}\right)}}
\newcommand{\totalvardist}[2]{\totalvardistrestr[]{#1}{#2}}
\newcommand{\chisquare}[2]{\operatorname{d_{\chi^2}}\mleft(#1,#2\mright)}
\newcommand{\dist}[2]{\operatorname{dist}\mleft({#1, #2}\mright)}
\newcommand{\kldiv}[2]{{D\mleft({#1 \| #2}\mright)}}

%
\newcommand\restr[2]{{%
  \left.\kern-\nulldelimiterspace %
  #1 %
  \vphantom{\big|} %
  \right|_{#2} %
  }}

%
\newcommand{\proba}{\Pr}
\newcommand{\probaOf}[1]{\proba\mleft[\, #1\, \mright]}
\newcommand{\bPr}[1]{\Pr\mleft[#1\mright]}
\newcommand{\probaCond}[2]{\proba\mleft[\, #1 \;\middle\vert\; #2\, \mright]}
\newcommand{\probaDistrOf}[2]{\proba_{#1}\mleft[\, #2\, \mright]}

%
\newcommand{\supp}[1]{\operatorname{supp}\mleft(#1\mright)}

%
\newcommand{\expect}[1]{\mathbb{E}\!\left[#1\right]}
\newcommand{\expectCond}[2]{\mathbb{E}\!\left[\, #1 \;\middle\vert\; #2\, \right]}
\newcommand{\shortexpect}{\mathbb{E}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\bEE}[1]{\shortexpect{\mleft[#1\mright]}}
\newcommand{\bE}[2]{\shortexpect_{#1}{\mleft[#2\mright]}}


%
\newcommand{\uniform}{\ensuremath{\mathbf{u}}}
\newcommand{\uniformOn}[1]{\ensuremath{\uniform_{ #1 } }}
\newcommand{\geom}[1]{\ensuremath{\operatorname{Geom}\!\left( #1 \right)}}
\newcommand{\bernoulli}[1]{\ensuremath{\operatorname{Bern}( #1 ) }}
\newcommand{\binomial}[2]{\ensuremath{\operatorname{Bin}\!\left( #1, #2 \right)}}
\newcommand{\poisson}[1]{\ensuremath{\operatorname{Poisson}\!\left( #1 \right) }}
\newcommand{\gaussian}[2]{\ensuremath{ \mathcal{G}\!\left(#1,#2\right) }}
\newcommand{\gaussianpdf}[2]{\ensuremath{ g_{#1,#2}}}
\newcommand{\betadistr}[2]{\ensuremath{ \operatorname{Beta}\!\left( #1, #2 \right) }}

%
\newcommand{\mutualinfo}[2]{ I(#1\wedge #2) }
\newcommand{\entropy}[1]{ H(#1) }
\newcommand{\condentropy}[2]{ \entropy{#1\mid#2} }

%
\newcommand{\norm}[1]{\lVert#1{\rVert}}
\newcommand{\normone}[1]{{\norm{#1}}_1}
\newcommand{\normtwo}[1]{{\norm{#1}}_2}
\newcommand{\normfour}[1]{{\norm{#1}}_4}
\newcommand{\norminf}[1]{{\norm{#1}}_\infty}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\dabs}[1]{\lvert #1 \rvert}
\newcommand{\dotprod}[2]{ \left\langle #1,\xspace #2 \right\rangle } 			%
\newcommand{\ip}[2]{\dotprod{#1}{#2}} 			%

\newcommand{\vect}[1]{\mathbf{#1}} 			%

%
\newcommand{\clg}[1]{\left\lceil #1 \right\rceil}
\newcommand{\flr}[1]{\left\lfloor #1 \right\rfloor}

%
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\C}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\N}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\cont}[1]{\ensuremath{\mathcal{C}^{#1}}}

%
\newcommand{\lp}[1][1]{\ell_{#1}}

%
\DeclareMathOperator{\convolution}{\ast}

\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\h}{\mathbf{h}}

%
\newcommand{\cE}{\mathcal{E}} \newcommand{\cI}{\mathcal{I}}
\newcommand{\cP}{\mathcal{P}} \newcommand{\cS}{\mathcal{S}}
\newcommand{\cX}{\mathcal{X}} \newcommand{\cY}{\mathcal{Y}}
\newcommand{\cW}{\mathcal{W}} \newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cA}{\mathcal{A}} \newcommand{\cC}{\mathcal{C}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cM}{\mathcal{M}}

%
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\bool}{\{-1,+1\}}

\newcommand{\chisquaredec}{\chi^{(2)}}
\newcommand{\ochisquaredec}{\overline{\chi}^{(2)}}
\newcommand{\uchisquaredec}{\underline{\chi}^{(2)}}


%
%
%
\newcommand{\referee}{\mathcal{R}\xspace}
%
\newcommand{\ab}{n} %
\newcommand{\numparts}{k}
\newcommand{\priv}{\rho} %
\newcommand{\dst}{\eps}     %
\newcommand{\parties}{n}
\newcommand{\loss}{l}     %
\newcommand{\Paren}[1]{\left(#1\right)}


\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\cf}{\textit{cf.}}



%
%


%
\newcommand{\parti}[1]{\mathrm{parti}(#1)} %
\newcommand{\moms}{r}
\newcommand{\sets}{S}
\newcommand{\sett}{T}
\newcommand{\maxint}{M}
\newcommand{\momvec}[2]{V^{#1,#2}}
\newcommand{\bucketsz}{k}
\newcommand{\mult}{\ell}
\newcommand{\closedist}{\mathbf{c}}
\newcommand{\fardist}{\mathbf{f}}
\newcommand{\refdist}{\mathbf{r}}
\newcommand{\elts}{s}
\newcommand{\eltt}{t}
\newcommand{\bucket}[2]{I_{#1,#2}}

\newcommand{\closefam}{\mathcal{C}}
\newcommand{\farfam}{\mathcal{F}}
\newcommand{\unndist}[2]{\mathrm{unndist}(#1,#2)}

